UniTalker: Scaling up Audio-Driven 3D Facial Animation through A Unified Model

Audio-driven 3D facial animation aims to map input audio to realistic facial motion. Despite significant progress, limitations arise from inconsistent 3D annotations, restricting previous models to training on specific annotations and thereby constraining the training scale. In this work, we present UniTalker, a unified model featuring a multi-head architecture designed to effectively leverage datasets with varied annotations. To enhance training stability and ensure consistency among multi-head outputs, we employ three training strategies, namely, PCA, model warm-up, and pivot identity embedding. To expand the training scale and diversity, we assemble A2F-Bench, comprising five publicly available datasets and three newly curated datasets. These datasets contain a wide range of audio domains, covering multilingual speech voices and songs, thereby scaling the training data from commonly employed datasets, typically less than 1 hour, to 18.5 hours. With a single trained UniTalker model, we achieve substantial lip vertex error reductions of 9.2% for BIWI dataset and 13.7% for Vocaset. Additionally, the pre-trained UniTalker exhibits promise as the foundation model for audio-driven facial animation tasks. Fine-tuning the pre-trained UniTalker on seen datasets further enhances performance on each dataset, with an average error reduction of 6.3% on A2F-Bench. Moreover, fine-tuning UniTalker on an unseen dataset with only half the data surpasses prior state-of-the-art models trained on the full dataset. The code and dataset are available at the project page https://github.com/X-niper/UniTalker.

==> figures/User_study_table_and_data_correlation_figure.tex <==
% \begin{minipage}[t]{0.5\textwidth}
%     \begin{table}[ht]
%     \centering
%     \caption{User study results. The numbers in the table mean UniTalker selection ratio.}
%     \label{tab:user_study}
%     \small
%     \begin{tabular}{l | c c c}
%     \toprule
%     \textbf{Method} & \textbf{Realistic} &  \textbf{Lip Sync} & \textbf{Emotion} \\
%     \midrule
%     Ours vs. FaceFormer &  74.7\% & 76.6\% & 78.2\% \\
%     Ours vs. CodeTalker  & 71.8\% & 77.1\% & 80.7\% \\
%     Ours vs. SelfTalker  & 72.5\% & 75.0\% & 82.1\% \\
%     \bottomrule
%     \end{tabular}
%     \end{table}
% \end{minipage}

% \hfill\begin{minipage}[t]{0.45\textwidth}
%     \begin{figure}
%     \includegraphics[width=\textwidth]{figures/images/heatmap_2314.pdf}
%     \caption{Comparison between finetuning Wav2Vec2-XLSR-53~\cite{Wav2Vec2_XLSR_53} and finetuning UniTalker-L-[D1-D7] on D0, \ie, BIWI. The x-axis is in log-scale. }
%     \label{fig:miniBIWI_transfer_compare}
%     \end{figure}
% \end

\begin{figure}[htb]
\begin{minipage}[]{0.38\textwidth}
\small 
% \centering
% \begin{tabular}{l | c c c}
%     \toprule
%     \textbf{Method} & \textbf{Realistic} &  \textbf{Lip Sync} & \textbf{Emotion} \\
%     \midrule
%     Ours vs. FaceFormer &  74.7\% & 76.6\% & 78.2\% \\
%     Ours vs. CodeTalker  & 71.8\% & 77.1\% & 80.7\% \\
%     Ours vs. SelfTalker  & 72.5\% & 75.0\% & 82.1\% \\
%     \bottomrule
% \end{tabular}
\captionof{table}{User study results. The numbers represent the support rate for UniTalker over its competitors, in terms of realism, lip-sync and facial emotion.}
\begin{tabular}{l | l | c }
    \toprule
    \textbf{Method} & \textbf{Question} & \textbf{Rate} \\
    \midrule
    \multirow{3}{*}{FaceFormer} & Realism &  74.7 \% \\
    & LipSync &  76.6 \% \\
    & Emotion &  78.2 \% \\
    \hline
    \multirow{3}{*}{CodeTalker} & Realism &  71.8 \% \\
    & LipSync &  77.1 \% \\
    & Emotion &  80.7 \% \\
    \hline
    \multirow{3}{*}{SelfTalk} & Realism &  72.5 \% \\
    & LipSync &  75.0 \% \\
    & Emotion &  82.1 \% \\
    \bottomrule
\end{tabular}
\label{tab:user_study}
% \captionof{table}{User study results. The numbers represent the support rate for UniTalker over its competitors.}
\end{minipage}
% 
 \hfill\begin{minipage}[]{0.61\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{figures/images/heatmap_2314.pdf}
\caption{
% Evaluation of each model trained on a single dataset across multiple test sets. 
% The row label denotes the training dataset. The column label denotes the test dataset.
The value at $j$th row and $i$th column $E_{[Dj]}^{i}$ indicates the performance gap on Di test set between UniTalker-[Dj] and UniTalker-[D0-D7].}
\label{fig:ex_heatmap}
\end{minipage}
\end{figure}

==> figures/annotation_transfer_figure_and_table.tex <==
\begin{figure}[tb]
\centering
 \begin{minipage}[t]{0.53\textwidth}
    \include{figures/miniBIWI_transfer}
    % \includegraphics[width=\linewidth]{figures/images/pie_compare_1118.pdf}
    % \caption{\textbf{Effect of PIE.} Without PIE, the model generates unnatural facial motion when input identity and output annotation mismatch.}
    % \label{fig:pivot_embedding_compare}
    \input{figures/miniBIWI_transfer}
 \end{minipage}
 \begin{minipage}[t]{0.45\textwidth}
    \centering
    % \input{tables/oneshot_vocaset_tuning}
    \include{tables/oneshot_vocaset_tuning}
    % \includegraphics[width=\linewidth]{figures/images/heatmap_half.pdf}
    % \caption{Relative LVD differences on each test dataset between a transferred model to transferred UniTalker-L-[D0,D7]}
    % \label{fig:ex_heatmap}
 \end{minipage}
\end{figure}

==> figures/dataset_correlation.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/images/heatmap_2314.pdf}
    \caption{Evaluation of each model trained on a single dataset across multiple test sets. The row label denotes the training dataset. The column label denotes the test dataset. The value at $j$th row and $i$th column is denoted by $E_{[Dj]}^{i}$, indicating the performance gap between UniTalker-[Dj] and UniTalker-[D0-D7].}
    % Relative LVE differences on each test dataset between a model trained on to transferred UniTalker-L-[D0,D7]
    % \todo{Revise the caption such that readers can understand without reading the main text, i.e., replacing ``transferred'' to something eaiser to understand}
    \label{fig:ex_heatmap}
\end{figure*}

==> figures/error_map.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/images/error_map_full.pdf}
  % \begin{subfigure}{0.0\linewidth}
  %   \label{subfig:mean of motion variation}
  % \end{subfigure}
  % \begin{subfigure}{0.0\linewidth}
  %   \label{subfig:std of motion variation}
  % \end{subfigure}
    \caption{\textbf{(a, b)} The temporal statistics (mean and standard deviation) of adjacent-frame motion variation within a sequence. \textbf{(c)} The mean of per-frame predicted-to-GT Euclidean distance within a sequence. \textbf{(d)} The standard deviation of facial motion within each training set.  The upper face of D1(VOCASET) shows little motion variation and is close to static
    }
    \label{fig:error map}
\end{figure}

==> figures/noUse_debug_figure.tex <==
\begin{figure}
 \includegraphics[width=0.4\linewidth]{figures/images/heatmap_2314.pdf}
 \caption{\texttt{none}}
\end{figure}

\begin{figure}
 \hfill\includegraphics[width=0.4\linewidth]{figures/images/heatmap_2314.pdf}
 \caption{\texttt{hfill}}
\end{figure}

\begin{figure}
 \begin{flushright}% or better \raggedleft see comments below
  \includegraphics[width=0.4\linewidth]{figures/images/heatmap_2314.pdf}
  \caption{\texttt{flushright}}
 \end{flushright}
\end{figure}

\begin{figure}
 \hfill\begin{minipage}{.5\textwidth}\centering
  \includegraphics[width=\linewidth]{figures/images/heatmap_2314.pdf}
  \caption{\texttt{minipage}}
 \end{minipage}
\end{figure}

==> figures/noUse_miniBIWI_transfer.tex <==
\begin{figure}[tb]
  \centering
  % \captionsetup{width=0.49\textwidth}
  \includegraphics[width=0.49\linewidth]{figures/images/miniBIWI_transfer.pdf}
  \caption{Comparison between finetuning Wav2Vec2-XLSR-53~\cite{Wav2Vec2_XLSR_53} on BIWI(D0) and finetuning UniTalker-L-[D1-D7] on BIWI(D0)\todo{Highlight the x-axis is log-scale?}}
  \label{fig:miniBIWI_transfer_compare}
\end{figure}

==> figures/noUse_pivot_id.tex <==
\begin{figure}[h]
  \centering
  % \captionsetup{width=0.49\textwidth}
  \includegraphics[width=0.49\linewidth]{figures/images/pie_compare_1118.pdf}
  \caption{\textbf{Effect of PIE.} Without PIE, the model generates unnatural facial motion when input identity and output annotation mismatch.}
  \label{fig:pivot_embedding_compare}
%  \end{minipage}
%  \begin{minipage}[t]{0.45\textwidth}
%     \input{figures/miniBIWI_transfer}
%     % \centering
%     % \includegraphics[width=\linewidth]{figures/images/heatmap_2314.pdf}
%     % \caption{Relative LVD differences on each test dataset between a transferred model to transferred UniTalker-L-[D0,D7]
%     % \todo{Revise the caption such that readers can understand without reading the main text, i.e., replacing ``transferred'' to something eaiser to understand}
%     % }
%     % \label{fig:ex_heatmap}
%  \end{minipage}
%  \begin{minipage}[t]{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/images/heatmap_2314.pdf}
%     \caption{Relative LVD differences on each test dataset between a transferred model to transferred UniTalker-L-[D0,D7]
%     \todo{Revise the caption such that readers can understand without reading the main text, i.e., replacing ``transferred'' to something eaiser to understand}
%     }
%     \label{fig:ex_heatmap}
%  \end{minipage}
\end{figure}

==> figures/noUse_pivot_id_and_dataset_correlation_old.tex <==
\begin{figure*}[h]
\centering
% \captionsetup{width=0.53\textwidth}
 \begin{minipage}[t]{0.53\textwidth}
    \includegraphics[width=\linewidth]{figures/images/pie_compare_1118.pdf}
    \caption{\textbf{Effect of PIE.} Without PIE, the model generates unnatural facial motion when input identity and output annotation mismatch.}
    \label{fig:pivot_embedding_compare}
 \end{minipage}
 \begin{minipage}[t]{0.45\textwidth}
    \input{figures/miniBIWI_transfer}
    % \centering
    % \includegraphics[width=\linewidth]{figures/images/heatmap_2314.pdf}
    % \caption{Relative LVD differences on each test dataset between a transferred model to transferred UniTalker-L-[D0,D7]
    % \todo{Revise the caption such that readers can understand without reading the main text, i.e., replacing ``transferred'' to something eaiser to understand}
    % }
    % \label{fig:ex_heatmap}
 \end{minipage}
 \begin{minipage}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/images/heatmap_2314.pdf}
    \caption{Relative LVD differences on each test dataset between a transferred model to transferred UniTalker-L-[D0,D7]
    \todo{Revise the caption such that readers can understand without reading the main text, i.e., replacing ``transferred'' to something eaiser to understand}
    }
    \label{fig:ex_heatmap}
 \end{minipage}
\end{figure*}

==> rebuttal_figures/fig_error_map.tex <==
\vspace{-4mm}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\linewidth]{rebuttal_figures/images/eccv_rebuttal_fig1.pdf}
  % \caption{\textbf{UniTalker architecture.} UniTalker adopts vertices PCA to balance the annotation dimension across datasets, uses decoder warm-up to stablize training, and develops a pivot identity embedding to mitigate dataset bias. Loss is calculated on vertices to balance the training for each decoder head.}
  \label{rebut_fig:error_map}
\end{figure}
\vspace{-6mm}


==> rebuttal_figures/fig_zoomed_in_multihead.tex <==
\vspace{-3mm}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{rebuttal_figures/images/ECCV-zoomed-in-multihead.pdf}
  \label{rebut_fig:multihead design}
\end{figure}
\vspace{-5mm}

==> rebuttal_tables/more_metric_compare.tex <==
\vspace{-4mm}
\begin{table}[h]
\centering
% \caption{More Metric.}
\label{tab:rebuttal_more_metric}
% \footnotesize
\tiny 
\begin{tabular}{p{0.8cm}|p{0.7cm}p{0.7cm}p{0.7cm}|p{0.75cm}p{0.75cm}p{0.75cm}}
\hline
\multirow{3}{*}{\textbf{Method}} & \multicolumn{3}{c|}{BIWI-Test-A} & \multicolumn{3}{c}{VOCA-Test} \\ & \textbf{MVE} $\downarrow$ & \textbf{UFVE} $\downarrow$ & \textbf{FDD} $\downarrow$ & \textbf{MVE} $\downarrow$ & \textbf{UFVE} $\downarrow$ & \textbf{FDD} $\downarrow$ \\
% & \textbf{$\times 10^{-3}$} & \textbf{$\times 10^{-3}$} & \textbf{$\times 10^{-5}$} &  \textbf{$\times 10^{-3} m$} & \textbf{$\times 10^{-3} m$} & \textbf{$\times 10^{-7} m^{2}$ } \\
& \textbf{$\times 10^{-3}$} & \textbf{$\times 10^{-3}$} & \textbf{$\times 10^{-5}$} &  \textbf{$\times 10^{-3} m$} & \textbf{$\times 10^{-3} m$} & \textbf{$\times 10^{-7} m^{2}$ } \\
% \vspace{-1mm}
% \end{tabular}
% \scriptsize
% \begin{tabular}{p{1.1cm}|p{0.7cm}p{0.7cm}p{0.7cm}|p{0.7cm}p{0.7cm}p{0.7cm}}
\hline
FF~[13]       & 7.2750  & 6.9081 & 4.0062   & 0.6364 & 0.4972 & 2.4812 \\
CT~[39]      & 7.3784  & 7.0050 & 4.2147   & 0.5750 & 0.4708 & 1.2594    \\
ST~[28]        & 6.9152  & 6.5428 & \textbf{3.5851} & 0.5665 & 0.4805 & \textbf{1.0511}  \\
FD~[34]    & 6.8088  & 6.6220 &  3.9101  & 0.5768 & 0.4772 & 1.7335 \\
\hline
B-[D*]                            & 6.8948  & 6.6277 & 4.6789 & 0.5695 & 0.4829 & 1.2115 \\
B-[D0-D7]                         & 6.6458  & 6.3774 & 5.0438 & \textbf{0.5338} & \textbf{0.4494} & 1.3962 \\
L-[D0-D7]                         & \textbf{6.4166} & \textbf{6.1483} & 5.2307 & 0.5524 & 0.4756 & 1.5206  \\
\hline
\end{tabular}
\end{table}
\vspace{-5mm}

==> rebuttal_tables/more_metric_compare2.tex <==
\vspace{-3mm}
\begin{table}[h]
\centering
% \caption{More Metric.}
\label{tab:rebuttal_more_metric}
% \footnotesize
\tiny 
\begin{tabular}{p{0.8cm}|p{0.7cm}p{0.7cm}p{0.7cm}|p{0.75cm}p{0.75cm}p{0.75cm}}
\hline
\multirow{3}{*}{\textbf{Method}} & \multicolumn{3}{c|}{BIWI-Test-A} & \multicolumn{3}{c}{VOCA-Test} \\ & \textbf{MVE} $\downarrow$ & \textbf{UFVE} $\downarrow$ & \textbf{FDD} $\downarrow$ & \textbf{MVE} $\downarrow$ & \textbf{UFVE} $\downarrow$ & \textbf{FDD} $\downarrow$ \\
% & \textbf{$\times 10^{-3}$} & \textbf{$\times 10^{-3}$} & \textbf{$\times 10^{-5}$} &  \textbf{$\times 10^{-3} m$} & \textbf{$\times 10^{-3} m$} & \textbf{$\times 10^{-7} m^{2}$ } \\
& \textbf{$\times 10^{-4}$} & \textbf{$\times 10^{-4}$} & \textbf{$\times 10^{-5}$} &  \textbf{$\times 10^{-5} m^2$} & \textbf{$\times 10^{-6} m^2$} & \textbf{$\times 10^{-7} m^{2}$ } \\
% \vspace{-1mm}
% \end{tabular}
% \scriptsize
% \begin{tabular}{p{1.1cm}|p{0.7cm}p{0.7cm}p{0.7cm}|p{0.7cm}p{0.7cm}p{0.7cm}}
\hline
FF~[13]       & 6.2313  & 3.1942 & 4.0062   & 2.9167 & 2.5571 & 2.4812 \\
CT~[39]      & 5.9907  & 3.1566 & 4.2147   & 2.9766 & 2.5148 & 1.2594    \\
ST~[28]        & 5.0942  & 2.6673 & \textbf{3.5851} & 2.9810 & 2.4270 & \textbf{1.0511}  \\
FD~[34]    & 5.5836  & 2.8966 &  3.9101  & 2.8310 & 2.6545 & 1.7335 \\
\hline
B-[D*]                            & 5.4972  & 2.9278 & 4.6789 & 2.9764 & 3.0310 & 1.2115 \\
B-[D0-D7]                         & 5.1230  & 2.7369 & 5.0438 & 2.7006 & \textbf{2.2633} & 1.3962 \\
L-[D0-D7]                         & \textbf{4.8863} & \textbf{2.5874} & 5.2307 & \textbf{2.5520} & 2.5242 & 1.5206  \\
\hline
\end{tabular}
\end{table}
\vspace{-4mm}

==> supp_sec/0_overview.tex <==
\section{Overview}
% Give an overview of the Supp

This supplementary materials provide additional information regarding the related works, model design, experiment results and the limitations of this work.

In section \ref{sec:supp_related_works_dataset}, we introduce the distinctions and connections between vertex-based annotations and parameter-based facial motion annotations. We introduce the conventional re-topology technique, which transforms meshes from one topology to another using linear transformations. This elucidates our rationale for selecting a linear layer as the decoder head in our model. 
% 
In section \ref{sec:supp_related_works_regression_autoregression}, we review the utilization of autoregressive and regressive models in recent studies focusing on audio-driven 3D facial motion. 
% 
In section \ref{sec:supp_IPCA_and_DW}, we investigate the feasibility of implementing the decoder warm-up strategy independently, without the need for adopting the IPCA strategy. We discuss more functionality of IPCA in this section. 
% 
In section \ref{sec:supp_PIE}, we discuss more on the pivot identity embedding (PIE) strategy. Additionally, we explore alternative solutions to address the issue of dataset bias leakage.
% 
In section \ref{sec:supp_dataset_description}, we show the details of the datasets used in the experiments. 
% 
In section \ref{sec:supp_experiment_details}, we show the details of the experimental settings. 
% 
In section \ref{sec:supp_frequency_adaptor_position}, we present a comparative analysis of various position choices of the frequency adaptor.
% 
In section \ref{sec:dataset_contribution_analysis}, we present additional analysis focusing on the contribution of different datasets to the overall model performance. This analysis aims to clarify the importance of incorporating mixed datasets to train a foundation model.
% 
In section \ref{sec:supp_transfer_to_tiny},  we showcase UniTalker's ability to transfer to unseen annotation conventions, even with minimal training data, including just a few audio-visual pairs or even one pair.
% 
% we show more results on annotation transfer to demonstrate the necessity of mixed datasets to build a foundation model. Firstly, we show that tuning the decoder part of the UniTalker-L-[D0-D7] model on a single dataset yields better performance that directly training the model on the dataset does. Secondly, to show that tuning a UniTalker model on an unseen dataset can greatly reduce the requirement of data size, we tune the decoder of UniTalker-L-[D1-D7] on D0 dataset and show the precision to data size relation. Thirdly, we utilise the mini-dataset transfer method explained in Section \missref to demonstrate that our model can transfer to new conventions with extremely small dataset. We show the visual results in the attached video.
% 
In section \ref{sec:supp_user_study}, we present a user study that qualitatively compares our work with previous state-of-the-art approaches.
% 
In section \ref{sec:supp_future_work}, we expose the limitations of UniTalker and outline future plans to address them.

==> supp_tables/UniTalker_and_vanilla_model.tex <==
\begin{table}[]
\centering
\caption{\textbf{Effect of frequency adaptor position.} Pos-0 means that the frequency adaptor is placed between the TCN and transformer in the audio encoder. Pos-1 means that the frequency adaptor is placed behind the transformer. The metric is LVE.
% 
LVE is in ${10^{-4}}$ for D0, ${10^{-6}}$ ${m^{2}}$ for D1-D3 and ${10^{-5}}$ ${m^{2}}$ for D4-D7
} 
\label{supp_tab:effect_of_frequency_adaptor}
\small
\begin{tabular}{l | c c c c c c c c}
\toprule
\textbf{Method}  &  \textbf{D0} & \textbf{D1} & \textbf{D2} & \textbf{D3} & \textbf{D4} & \textbf{D5} & \textbf{D6} & \textbf{D7} \\
\midrule
\textbf{L-[D*]} &  4.279 & 9.153 & 8.881 & \textbf{8.445} & 1.370 & \textbf{2.040} & \textbf{1.043} & 1.235 \\
\textbf{Vanilla}  &    4.031 &      8.415 &          9.049 &           9.342 &             1.448 &               2.041 &       1.092 &             1.276  \\
\textbf{UniTalker} &    \textbf{3.859} &        \textbf{8.303} &          \textbf{8.648} &           8.991 &             \textbf{1.326} &               2.056 &       1.145 &             \textbf{1.211}  \\
\bottomrule
\end{tabular}
\end{table}


==> tables/LVD_comparison_between_single_and_D0_D7.tex <==
\begin{table}[h]
% \footnotesize
\scriptsize
% \tiny
%\setlength\tabcolsep{2pt}
\centering
\caption{Quantitative comparison between single dataset training and mixed dataset training. The metric is LVD (mm). B and L represents using base and large wav2vec 2.0 model, respectively. [single] indicates the model is trained on each single dataset. [D0-D7] refers to using all datasets for training. L$^*$ desigates fine-tuning on each dataset.}
\label{tab:ablation}
\begin{tabular}{l | c c c c c c c c}
\toprule
{\textbf{Method}} & \textbf{D0}  & \textbf{D1}  & \textbf{D2} & \textbf{D3} & \textbf{D4} & \textbf{D5}  & \textbf{D6} &\textbf{D7} \\
 % & ($mm$)  & ($mm$) & ($mm$) & ($mm$) & ($mm$) & ($mm$) & ($mm$) & ($mm$)\\
\midrule
% precision: .4f
% B-[Single]      & 3.8885   & 2.7090     & 2.8992    & 2.5747 & 3.1972 & 3.9628 & 2.8121 & 3.0323 \\
% B-[D0-D7]       & 3.7645\textcolor{Green}{$\downarrow_{3.2\%}$}   & 2.8046\textcolor{Red}{$\uparrow_{3.5\%}$}     & 2.8067\textcolor{Green}{$\downarrow_{3.2\%}$}    & 2.6960\textcolor{Red}{$\uparrow_{4.7\%}$} & 3.1942\textcolor{Green}{$\downarrow_{0.1\%}$} & 4.0748\textcolor{Red}{$\uparrow_{2.8\%}$} & 3.0050\textcolor{Red}{$\uparrow_{6.9\%}$} & 3.0280\textcolor{Green}{$\downarrow_{0.1\%}$} \\
% \hline
% L-[Single]      & 3.7574   & 2.7442     & 2.6572    & 2.4898 & 3.0089 & 3.9130 & 2.6493 & 2.8234 \\
% L-[D0-D7]       & 3.5000\textcolor{Green}{$\downarrow_{6.9\%}$}   & 2.5940\textcolor{Green}{$\downarrow_{5.5\%}$}     & 2.6029\textcolor{Green}{$\downarrow_{2.0\%}$} & 2.5799\textcolor{Red}{$\uparrow_{3.6\%}$} & 2.9914\textcolor{Green}{$\downarrow_{0.6\%}$} & 3.9385\textcolor{Red}{$\uparrow_{0.7\%}$} & 2.7641\textcolor{Red}{$\uparrow_{4.3\%}$} & 2.8442\textcolor{Red}{$\uparrow_{0.7\%}$} \\
% L$^*$-[D0-D7]     & 3.4779\textcolor{Green}{$\downarrow_{7.4\%}$}   & 2.5297\textcolor{Green}{$\downarrow_{7.8\%}$} & 2.6051\textcolor{Green}{$\downarrow_{2.0\%}$} & 2.4775\textcolor{Green}{$\downarrow_{0.5\%}$} & 2.9381\textcolor{Green}{$\downarrow_{2.4\%}$}   & 3.7614\textcolor{Green}{$\downarrow_{3.9\%}$}   &  2.5510\textcolor{Green}{$\downarrow_{3.7\%}$}   &  2.7554(\textcolor{Green}{$\downarrow_{2.4\%}$}  \\
% precision: .3f
B-[Single]      & 3.889   & 2.709     & 2.899    & 2.575 & 3.197 & 3.963 & 2.812 & 3.032 \\
B-[D0-D7]       & 3.765\textcolor{Green}{$\downarrow_{3.2\%}$}   & 2.805\textcolor{Red}{$\uparrow_{3.5\%}$}     & 2.807\textcolor{Green}{$\downarrow_{3.2\%}$}    & 2.696\textcolor{Red}{$\uparrow_{4.7\%}$} & 3.194\textcolor{Green}{$\downarrow_{0.1\%}$} & 4.075\textcolor{Red}{$\uparrow_{2.8\%}$} & 3.005\textcolor{Red}{$\uparrow_{6.9\%}$} & 3.028\textcolor{Green}{$\downarrow_{0.1\%}$} \\
\midrule
L-[Single]      & 3.757   & 2.744     & 2.657    & 2.490 & 3.009 & 3.913 & 2.649 & 2.823 \\
L-[D0-D7]       & 3.500\textcolor{Green}{$\downarrow_{6.9\%}$}   & 2.594\textcolor{Green}{$\downarrow_{5.5\%}$}     & 2.603\textcolor{Green}{$\downarrow_{2.0\%}$} & 2.580\textcolor{Red}{$\uparrow_{3.6\%}$} & 2.991\textcolor{Green}{$\downarrow_{0.6\%}$} & 3.939\textcolor{Red}{$\uparrow_{0.7\%}$} & 2.764\textcolor{Red}{$\uparrow_{4.3\%}$} & 2.844\textcolor{Red}{$\uparrow_{0.7\%}$} \\
L$^*$-[D0-D7]     & 3.478\textcolor{Green}{$\downarrow_{7.4\%}$}   & 2.530\textcolor{Green}{$\downarrow_{7.8\%}$} & 2.605\textcolor{Green}{$\downarrow_{2.0\%}$} & 2.478\textcolor{Green}{$\downarrow_{0.5\%}$} & 2.938\textcolor{Green}{$\downarrow_{2.4\%}$}   & 3.761\textcolor{Green}{$\downarrow_{3.9\%}$}   &  2.551\textcolor{Green}{$\downarrow_{3.7\%}$}   &  2.755\textcolor{Green}{$\downarrow_{2.4\%}$}  \\
\bottomrule
\end{tabular}
\end{table}

==> tables/LVE_MVE_FDDcomparison.tex <==
\begin{table}[t]
\centering
\caption{Quantitative evaluation on BIWI and VOCASET. 
% Note that SelfTalk uses large wav2vec 2.0 as audio encoder by default.
% FaceDiffuser uses HuBERT audio encoder.
[D*] indicates D0(BIWI) and D1(VOCASET) for BIWI-Test-A and VOCA-Test, respectively.
% [D0-D4] represents the combination of all 5 English datasets, ranging from D0 to D4.
[D0-D7] indicates training on A2F-Bench.
Params refers to the trainable parameters.}
\label{tab:LVE_MVE_FDD_biwi_vocaset}
% \small
\scriptsize 
\begin{tabular}{l|cccccc|cccccc}
\toprule
% BIWI-Test-A
\multirow{3}{*}{\textbf{Method}} & \multicolumn{6}{c|}{BIWI-Test-A} & \multicolumn{6}{c}{VOCA-Test} \\
& \textbf{LVE} $\downarrow$ & \textbf{MVE} $\downarrow$ & \textbf{UFVE} $\downarrow$ & \textbf{FDD} $\downarrow$ &\textbf{Params} & \textbf{Time} $\downarrow$ & \textbf{LVE} $\downarrow$ & \textbf{MVE} $\downarrow$ & \textbf{UFVE} $\downarrow$ & \textbf{FDD} $\downarrow$ & \textbf{Params} & \textbf{Time} $\downarrow$ \\
 & ($\times 10^{-4}$) & ($\times 10^{-3}$) & ($\times 10^{-3}$) & ($\times 10^{-5}$) & ($M$) & ($s$) & ($\times 10^{-5}$ $m^{2}$) & ($\times 10^{-3}$ $m$) & ($\times 10^{-3}$ $m$) & ($\times 10^{-7}$ $m^{2}$) & ($M$) & ($s$)\\
\midrule
FaceFormer~\cite{fan2022faceformer}  & 4.9836   &  109     & 0.705 & 1.1696   & 92      & 0.624\\
% FaceFormer-L~\cite{fan2022faceformer}  & 4.2141   &    \missvalue   & \missvalue & 1.1630   &   \missvalue    & \missvalue \\
CodeTalker~\cite{xing2023codetalker}  & 4.7914   &  561   & 4.4 & 1.1182   & 315      & 3.464 \\
% CodeTalker-L~\cite{xing2023codetalker}  & 4.9583   &  \missvalue   & \missvalue & 1.0099   & \missvalue     & \missvalue \\
SelfTalk~\cite{peng2023selftalk}  & 4.2485   &  539    & 0.071 & 0.9626   & 450     & 0.053 \\
FaceDiffuser~\cite{stan2023facediffuser}  & 4.2985  &  189  & 16.50 & 0.9684  & 89     & 13.08 \\
\hline
UniTalker-B-[D*] & 4.3681 & 92 & 0.024 & 0.9381 & 92 & 0.022 \\
% UniTalker-B-[D0-D4] & 4.4515 & 92 & 0.024 & 0.9241 & 92 & 0.022 \\
UniTalker-B-[D0-D7] & \underline{4.0804} & 92 & 0.024 & \textbf{0.8136} & 92 & 0.022 \\
% UniTalker-[D*] & 4.2790 & 313 & 0.054 & 0.9153 & 313 & 0.053 \\
% Preprocess-L-[D0-D2] & - & - & - & 0.8240 & 316 & 0.053 \\
% UniTalker-L-[D0-D2] & 4.0783 & 313 & 0.054 & \textbf{0.7924} & 313 & 0.053 \\
% Preprocess-L-[D0-D7] & - & - & - & 0.8906 & 316 & 0.053 \\
UniTalker-L-[D0-D7] & \textbf{3.8587} & 313 & 0.054 & \underline{0.8303} & 313 & 0.053 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/LVE_comparison_BIWI_vocaset.tex <==
\begin{table}[ht]
\centering
\caption{Quantitative evaluation results on BIWI-Test-A and VOCA-Test. For UniTalker, B and L represents using base and large wav2vec 2.0 model, respectively.
Note that SelfTalk uses large wav2vec 2.0 as audio encoder by default. FaceDiffuser uses HuBERT audio encoder.
[D*] indicates D0(BIWI) and D1(VOCA-Test) for BIWI-Test-A and VOCA-Test, respectively.
[D0-D4] represents the combination of all 5 English datasets, ranging from D0 to D4.
[D0-D7] refers to using all datasets for training. Parameters refer to the trainable parameters in each model.}
\label{tab:LVE_biwi_vocaset}
\small
\begin{tabular}{l|ccc|ccc}
\toprule
% BIWI-Test-A
\multirow{3}{*}{\textbf{Method}} & \multicolumn{3}{c|}{BIWI-Test-A} & \multicolumn{3}{c}{VOCA-Test} \\ & \textbf{LVE} $\downarrow$ & \textbf{Parameters} & \textbf{Time} & \textbf{LVE} $\downarrow$ & \textbf{Parameters} & \textbf{Time} \\
 & ($\times 10^{-4}$) & ($M$) & ($s$) & ($\times 10^{-5}$) & ($M$) & ($s$)\\
\midrule
FaceFormer-B~\cite{fan2022faceformer}  & 4.9836   &  109     & 0.705 & 1.1696   & 92      & 0.624\\
FaceFormer-L~\cite{fan2022faceformer}  & 4.2141   &    \missvalue   & \missvalue & 1.1630   &   \missvalue    & \missvalue \\
CodeTalker-B~\cite{xing2023codetalker}  & 4.7914   &  561   & 4.4 & 1.1182   & 315      & 3.464 \\
CodeTalker-L~\cite{xing2023codetalker}  & 4.9583   &  \missvalue   & \missvalue & 1.0099   & \missvalue     & \missvalue \\
SelfTalk~\cite{peng2023selftalk}  & 4.2485   &  539    & 0.0709 & 0.9626   & 450     & 0.053 \\
FaceDiffuser~\cite{stan2023facediffuser}  & 4.2985  &  539  & 16.4973 & 0.9684  & 450     & 26.1557 \\
\hline
UniTalker-B-[D*] & 4.815 & 92 & 0.024 & 0.9125 & 92 & 0.022 \\
% UniTalker-B-[D0-D4] & 4.4515 & 92 & 0.024 & 0.9241 & 92 & 0.022 \\
UniTalker-L-[D*] & 4.279 & 313 & 0.054 & 0.9153 & 313 & 0.053 \\
Preprocess-L-[D0-D2] & - & - & - & 0.8240 & 316 & 0.053 \\
UniTalker-L-[D0-D2] & 4.0783 & 313 & 0.054 & \textbf{0.7924} & 313 & 0.053 \\
Preprocess-L-[D0-D7] & - & - & - & 0.8906 & 316 & 0.053 \\
UniTalker-L-[D0-D7] & \textbf{3.8587} & 313 & 0.054 & 0.8304 & 313 & 0.053 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/LVE_comparison_less.tex <==
\begin{table}[t]
\centering
\caption{Quantitative evaluation on BIWI and VOCASET. 
% Note that SelfTalk uses large wav2vec 2.0 as audio encoder by default.
% FaceDiffuser uses HuBERT audio encoder.
[D*] indicates D0(BIWI) and D1(VOCASET) for BIWI-Test-A and VOCA-Test, respectively.
% [D0-D4] represents the combination of all 5 English datasets, ranging from D0 to D4.
[D0-D7] indicates training on A2F-Bench.
Params refers to the trainable parameters.}
\label{tab:LVE_biwi_vocaset}
% \small
\begin{tabular}{l|ccc|ccc}
\toprule
% BIWI-Test-A
\multirow{3}{*}{\textbf{Method}} & \multicolumn{3}{c|}{BIWI-Test-A} & \multicolumn{3}{c}{VOCA-Test} \\ & \textbf{LVE} $\downarrow$ & \textbf{Params} & \textbf{Time} $\downarrow$ & \textbf{LVE} $\downarrow$ & \textbf{Params} & \textbf{Time} $\downarrow$ \\
 & ($\times 10^{-4}$) & ($M$) & ($s$) & ($\times 10^{-5}$ $m^{2}$) & ($M$) & ($s$)\\
\midrule
FaceFormer~\cite{fan2022faceformer}  & 4.9836   &  109     & 0.705 & 1.1696   & 92      & 0.624\\
% FaceFormer-L~\cite{fan2022faceformer}  & 4.2141   &    \missvalue   & \missvalue & 1.1630   &   \missvalue    & \missvalue \\
CodeTalker~\cite{xing2023codetalker}  & 4.7914   &  561   & 4.4 & 1.1182   & 315      & 3.464 \\
% CodeTalker-L~\cite{xing2023codetalker}  & 4.9583   &  \missvalue   & \missvalue & 1.0099   & \missvalue     & \missvalue \\
SelfTalk~\cite{peng2023selftalk}  & 4.2485   &  539    & 0.071 & 0.9626   & 450     & 0.053 \\
FaceDiffuser~\cite{stan2023facediffuser}  & 4.2985  &  189  & 16.50 & 0.9684  & 89     & 13.08 \\
\hline
UniTalker-B-[D*] & 4.3681 & 92 & 0.024 & 0.9381 & 92 & 0.022 \\
% UniTalker-B-[D0-D4] & 4.4515 & 92 & 0.024 & 0.9241 & 92 & 0.022 \\
UniTalker-B-[D0-D7] & \underline{4.0804} & 92 & 0.024 & \textbf{0.8136} & 92 & 0.022 \\
% UniTalker-[D*] & 4.2790 & 313 & 0.054 & 0.9153 & 313 & 0.053 \\
% Preprocess-L-[D0-D2] & - & - & - & 0.8240 & 316 & 0.053 \\
% UniTalker-L-[D0-D2] & 4.0783 & 313 & 0.054 & \textbf{0.7924} & 313 & 0.053 \\
% Preprocess-L-[D0-D7] & - & - & - & 0.8906 & 316 & 0.053 \\
UniTalker-L-[D0-D7] & \textbf{3.8587} & 313 & 0.054 & \underline{0.8303} & 313 & 0.053 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/oneshot_vocaset_tuning.tex <==
\begin{table}[ht]
\centering
\caption{One-Shot Learning from Wav2Vec2-XLSR-53~\cite{Wav2Vec2_XLSR_53} and UniTalker-L-[D0,D2-D7] on VOCASET.}
\label{tab:one_shot_training}
\small
\begin{tabular}{l | c c }
\toprule
\textbf{Method} & \textbf{LVE / ${ \times \boldsymbol{1^{-5} m^2}}$} & \textbf{LVD / mm} \\
\midrule
Wav2Vec2-XLSR-53              & 3.4812   &  5.1479   \\
UniTalker-L-[D0,D2-D7]        & 2.2169   &  4.2043   \\
\bottomrule
\end{tabular}
\end{table}
